Scaling Large-scale GNN Training to Thousands of Processors on CPU-based Supercomputers

Graph Convolutional Networks (GCNs), particularly for large-scale graphs, are crucial across numerous domains. However, training distributed full-batch GCNs on large-scale graphs suffers from inefficient memory access patterns and high communication overhead. To address these challenges, we introduce \method{}, an efficient and scalable distributed GCN training framework tailored for CPU-powered supercomputers. Our contributions are threefold: (1) we develop general and efficient aggregation operators designed for irregular memory access, (2) we propose a hierarchical aggregation scheme that reduces communication costs without altering the graph structure, and (3) we present a communication-aware quantization scheme to enhance performance. Experimental results demonstrate that \method{} achieves a speedup of up to 6$\times$ compared with the SoTA implementations, and scales to 1000s of HPC-grade CPUs on the largest publicly available datasets, without sacrificing model convergence and accuracy. Moreover, due to the effective strong scaling of \method{}, we outperform SoTA GPU-based and CPU-based distributed full-batch GCN training frameworks, in absolute performance, for large-scale graphs.

==> 0.title.tex <==
% SuperGCN: General and Scalable Framework for GCN Training on CPU-powered Supercomputers\vspace{-10pt}
Scaling Large-scale GNN Training to Thousands of Processors on CPU-based Supercomputers
% \vspace{-10pt}
%\jiajun{SuperGCN: Effectively Scaling GCN Training to Thousands of Processors on CPU Supercomputers}\vspace{-10pt}
%Large-scale GCN Training on Supercomputers

==> 2-proposed_methods_lingqi.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{SuperGCN: General \& Scalable Distributed Full-batch GCNs Training Framework}


% \subsection{Overview of the SuperGCN}
% \zhuanghpdc{
% To achieve full-batch distributed GCN training, the original graph is partitioned into multiple subgraphs using the min-cut graph partitioning algorithm. Each subgraph is then assigned to a worker, and distributed training is conducted on these subgraphs. The two primary operations in GNN training are aggregation and MLP, with the main performance bottleneck arising from aggregation. In distributed training, aggregation is divided into two components: local node aggregation and remote node aggregation along cut edges across different workers.}

% \zhuanghpdc{
% In local node aggregation, each node aggregates the features of its neighboring nodes along edges. The random connectivity of the graph leads to numerous random memory accesses, reducing data reuse. This randomness also poses challenges to load balancing and parallelism. Furthermore, variations in input shapes and hardware characteristics (e.g., cache line size) make it difficult to design a general-purpose local aggregation kernel. Since local aggregation serves as the foundation for a scalable framework, optimizing it is critical. In the section on optimization techniques, we introduce methods to improve memory access patterns and enhance data reuse for better performance. Additionally, we address load balancing issues and propose a versatile inner kernel to further reduce memory access overhead.}

% \zhuanghpdc{
% In remote node aggregation, features of remote nodes residing on other workers are transferred along cut edges, resulting in significant communication overhead. This overhead becomes the primary scalability bottleneck as the number of workers increases. To address this, we propose a pre-post aggregation method to minimize the number of remote nodes, thereby reducing communication volume and enhancing communication efficiency. Furthermore, we design an efficient int2 quantization communication scheme with an accuracy recovery strategy to compress communication messages without compromising model accuracy. Together, these methods reduce communication time and improve the scalability of the framework.
% }


% Fig.~\ref{fig/method:overview_procedure} gives an overview of SuperGCN:
% \circled{1} The input graph is split into several subgraphs \zhuang{with the mini-cut graph partitioning method \emph{ParMetis}~\cite{karypis1997parmetis}}.
% %, and each subgraph is assigned to a worker. 
%     % \textcolor{blue}{A worker is a CPU (NUMA) node}.
% \circled{2} Each subgraph is divided into a local graph and a remote graph, with the remote graph containing boundary nodes. The remote graph is further divided into a pre-aggregation graph and a post-aggregation graph based on our proposed strategy described in \zhuang{Sec.~\ref{subsec:pre-post-aggregation}} 
% for reducing communication volume. 
% The pre-aggregation graph is exchanged between workers in this step. 
% \zhuangppopp{\circled{3} If label propagation is enabled, update the features of randomly selected nodes with their labels that have been embedded. The details of this step are in Sec~\ref{subsec:quantized_communication}.}
% \circled{4} Pre-aggregation is performed on the pre-aggregation graph using the optimized aggregation operators to collect boundary nodes' features.
% % that need to be transferred to other workers. 
% Furthermore, aggregation is done on the local graph to update the \zhuang{inner} nodes' features using the optimized operators. The optimization of aggregation operators is described in Sec.~\ref{subsec:index_add} and \ref{subsec:SPMM}.
%     % \item \emph{Random integer bits assigner} selects the quantized integer bit width for each boundary node's feature randomly from 2 bits, 4 bits, and 8 bits according to a predefined weight. 
% \circled{5} The boundary nodes' features acquired during the pre-aggregation phase are quantized to int2 and transmitted to other workers. % using the MPI Alltoallv collective~\cite{mpi40}. %\zhuang{Unlike some systems for small-scale GPU clusters that prefer to use P2P communication primitives, we apply the MPI  Alltoallv~\cite{mpi40} optimized for supercomputers to communicate.} 
%     % using the MPI library Alltoallv collective~\cite{mpi40}. 
% This communication is overlapped with the local aggregation in the preceding step. 
% After the communication, the received features from other workers are dequantized to FP32 \zhuang{with the received quantization parameters}. The details of this step are in Sec \ref{subsec:quantized_communication}.
% \circled{6} Post-aggregation is executed on the post-aggregation graph, and the received boundary nodes' features are integrated into the overall aggregation result. \zhuang{After this step, the aggregation in a GCN layer is completed. \circled{7} NN operation such as linear transform is performed.} Once this step is completed, the \zhuang{next GCN layer} will commence at the third step. This framework seamlessly applies to large-scale training of most message-passing-based GNN models, such as GraphSAGE~\cite{hamilton2017inductive}, GIN~\cite{xu2018powerful}, and GAT~\cite{velickovic2017graph}. 
% % For certain specialized GNNs with learnable message passing (e.g. GAT~\cite{velickovic2017graph}), 
% %although it exposes additional optimization opportunities while obtaining the weights for message passing, 
% % This framework can still be an efficient baseline for the message passing operation.
% \begin{comment}
% %\begin{figure}
% %    \centering
% %    \includegraphics[width=0.995\linewidth]{figures//method/overview_methods.pdf}
%     %\caption{Overview of our proposed system, includes %\emph{Node-level optimization} and \emph{Distributed %\label{fig/method:overview_methods}
% %\end{figure}

% % In this section, we introduce the proposed distributed GCNs training framework. An overview of our proposed method is depicted in Fig.~\ref{fig/method:overview_methods}. Once the graph is partitioned, we assign each subgraph to a CPU (NUMA) node prior to start the training process. In this data parallelism scheme, two types of performance bottlenecks emerge: aggregation operations within subgraphs and remote communication across subgraphs for boundary node exchange. To implement high-performance aggregation operation, we introduce \emph{Node-level optimization}, covering the optimization of aggregation operators Index\_add (Sec. \ref{subsec:index_add}) and SPMM (Sec. \ref{subsec:SPMM}). To minimize remote communication overhead during boundary node exchange, we present \emph{Distributed optimization} which includes pre- and post-aggregation (Sec. \ref{subsec:pre-post-aggregation}) and quantized communication (Sec. \ref{subsec:quantized_communication}). The integration of these proposed methods is outlined in Sec. \ref{subsec:procedure}.
% \end{comment}
% \subsection{Single processor optimizations}
% \lingqi{To achieve high performance in distributed GCN training, we design the training framework with a two-level optimization strategy: node-level optimizations (Sec.~\ref{sec:node_level_opt}) and distribute level optimizations (Sec.~\ref{sec:dist_level_opt}). We present a theoretical analysis (Sec.~\ref{sec:permodel_basic}) to demonstrate the effectiveness of our optimization approaches.

% }



% In full-batch GCNs training, there are two aggregation operators: tensor-related operation (\emph{Index\_add}) and matrix-related operation (\emph{Sparse Matrix-Martix Multiplication (SPMM)}). Since the matrix-related operation is similar to the inner kernel of tensor-related operation, in this subsection, we use tensor-related operation as an example (\emph{Index\_add}).

% \textbf{Main Process:} The process of \emph{Index\_add} operator is illustrated in Fig.~\ref{fig/method:index_add_origin}. In \emph{Index\_add}, the elements in the $src$ array are added to the $dst$ array at the positions specified by the corresponding elements in the $idx$ array.  This operator is employed to accumulate the received boundary nodes' feature to the local nodes. 

% \textbf{Optimizing Memory Access Pattern:} We improve the memory access pattern and locality of the $dst$ array in the original implementation. (1) \emph{Clustering and Sorting.} Initially, we cluster the rows in the $src$ array that need to be aggregated to the same row in the $dst$.
% \zhuanghpdc{Even though the order of accessing the rows of src is disrupted by sorting idx, since each row of src is still accessed sequentially and src only needs to be accessed once, there will not be much performance loss compared with the improvement of data reuse on $dst$.}
% This step is illustrated in Fig.~\ref{fig/method:index_add_sorted}.
% \zhuanghpdc{(2) Loop Reordering. We reorder the loops to deliver a chance for the following register-optimized kernel that improves data reuse on $dst$.}

% \textbf{Other optimizations:} We also optimize the operators by (1) 2D dynamic parallelism, (2) FLOPS-based load balance, and (3) efficient register kernel. 

\begin{comment}    
\textbf{Multi-threaded parallelism \  & load balance.} 
% In the original algorithm, threads are spawned on the cols (loop in line 4 of Algorithm \ref{alg:original_index_add}) of the $src$ array, which introduces the false sharing problem while the length of cols is insufficient. To address this issue, 
We propose a 2D dynamic parallelism strategy that involves spawning threads on both the rows and columns of the $src$ array (as illustrated in Fig.~\ref{fig/method:index_add_parallel}). On the row dimension, the overhead of atomic reduction is eliminated by sorting the $idx$ array \zhuang{in the proceeding step}. \zhuang{We assign rows to different threads based on the flops to achieve load balance.}
% To balance the load, we initially scan the $idx$ array to count the number of arithmetic operations on different rows and assign rows to different threads based on the count. 
% In cases where the length of the columns in the $src$ array is sufficiently large, we schedule some threads on this dimension. 
% The workload on this dimension is distributed evenly. 

% \input{listings/register_kernel_listing}
\textbf{\zhuanghpdc{General and} efficient register-optimized kernels based on code generation.} 
% To maximize the reuse of vector registers and cache lines, we propose a register kernel with the flexible shape $1 \times N$, where $N$ is determined by both the length of features and the size of the cache line.
\zhuanghpdc{To maximize the reuse of registers and cache lines, we propose a register kernel with the flexible shape $1 \times N$ with template-based code generation, where $N$ is determined by both the length of features and the size of the cache line. By aligning the kernel shape $N$ with the size of the cache line in different hardware, we can increase the reuse of the cache line and improve the effective bandwidth of our kernel.}
% We implement the register kernel using C++ templates and ARM predicate or Intel mask mechanism. This approach allows us to have a flexible kernel shape that adapts to the varying lengths of feature vectors resulting from different input data shapes and the different cache line sizes on various CPUs. 
As shown in Fig.~\ref{fig/method:index_add_reg}, we illustrate how $index\_add$ uses register kernel variants.

%\subsubsection{Optimization for aggregation operator Sparse Matrix-Matrix Multiplication (SPMM)}
\subsubsection{Optimizing aggregation operators for Sparse Matrix-Matrix Multiplication (SPMM)}
\label{subsec:SPMM}
 % SPMM involves multiplying a sparse matrix A with a dense matrix B to produce a dense matrix C. 
 \zhuangppopp{ \emph{SPMM} is used to collect and aggregate neighboring nodes' features. 
 We apply the methods proposed for \emph{Index\_add} to SPMM directly.}% \emph{SPMM} can be viewed as the core computation component of \emph{index\_add}. 
% After sorting the $idx$ array and clustering the rows in the $src$ matrix in \emph{index\_add}, \emph{SPMM} becomes equivalent to \emph{Index\_add}. Therefore, we apply similar optimization methods to \emph{SPMM}. 
\end{comment}

% After identifying the vertex set \(C\) of the minimum vertex cover (such as vertex 2 and 4 in Fig.~\ref{fig/method:minimum_vertex_cover}(c)), we construct pre- and post-aggregation graph based on this set, transforming the original edges communication into vertices communication on this set, thereby achieving the optimal communication volume.


\section{Algorithm-Invariant Communication Optimization}
\label{sec:proposed_methods}\label{sec:fram_work}
\wu{In distributed full-batch GCN training, communication performance is mainly influenced by graph partitioning (Section~\ref{sec:partition}) and the aggregation method.} We summarize the existing approaches for the aggregation (Section~\ref{subsec:pre-post-aggregation}) and introduce our hybrid aggregation strategy (Section~\ref{sec:hybridaggregation}). 


% During the aggregation stage, nodes must aggregate features from neighboring nodes located in other subgraphs along the cut edges. This boundary node exchange requires remote communication between subgraphs. In this section, we outline our proposed methods for mitigating the remote communication overhead during the boundary nodes exchange \wu{and provide a performance model to characterize the communication}.


\subsection{Graph partitioning algorithm selection}\label{sec:partition}
\zhuanghpdc{Regarding graph partitioning, we employ METIS~\cite{karypis1997parmetis} min-cut algorithm, which is widely adopted in popular GNN frameworks such as DGL~\cite{zheng2020distdgl}, PyG~\cite{fey2019pyg}, and so on~\cite{wan2022bns, wan2022pipegcn, peng2022sancus, ma2019neugraph, cai2021dgcl, wan2023adaptive, zhang2024sylvie}. METIS minimizes the total communication volume by minimizing the total number of cut edges. Additionally, it employs a hierarchical partitioning strategy to cluster the subgraphs, aiming to ensure that each subgraph communicates more data with its neighboring subgraphs than with remote ones. This locality property is beneficial for computing clusters and supercomputers where intra-node communication is significantly faster than inter-node communication.}

\subsection{\zhuang{Feature Aggregation Strategies: the traditional approaches}}
\label{subsec:pre-post-aggregation}
\label{sec:dist_level_opt}

% \subsubsection{Constructing Pre- and Post-aggregation Subgraph}
\begin{figure}[t]
    \centering
    \subfigure[$S_0$'s remote graph. 
    The transferred data volume is 5.
    ]{
        \begin{minipage}[b]{0.2\textwidth}
            \includegraphics[width=1\textwidth]{figures/method/complicated_original_graph.pdf}
        \end{minipage}
        \label{fig/method:complicated_original_graph}
    } \hspace{2mm}
    \subfigure[Convert to Pre-aggr graph. 
    The transferred data volume is 3.~\cite{md2021distgnn}
    ]{
        \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=1\textwidth]{figures/method/complicated_pre_graph_v1.pdf}
        \end{minipage}
    \label{fig/method:complicated_pre_graph}
    } 
    \\
    \subfigure[Convert to Post-aggr graph. 
    The transferred data volume is 3.~\cite{wan2022bns, wan2023adaptive, mostafa2022sequential, wan2022pipegcn}
    ]{
        \begin{minipage}[b]{0.2\textwidth}
            \includegraphics[width=1\textwidth]{figures/method/complicated_post_graph_v1.pdf}
        \end{minipage}
        \label{fig/method:complicated_post_graph}
    } \hspace{2mm}
    \subfigure[Ours : \zhuang{hybrid} of post-aggr and pre-aggr graph. 
    %The transferred data volume is 2 (Optimal).
    ]{
        \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=1\textwidth]{figures/method/complicated_optimal_graph_v1.pdf}
        \end{minipage}
    \label{fig/method:complicated_optimal_graph}
    } 
    \caption{Different strategies to reconstruct a remote graph.}
    \label{fig/method:complicated_graph}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%
After partitioning the graph, each subgraph is assigned to a \zhuang{worker}. By default, the subgraph will be divided into two parts: 
\begin{itemize}
    \item the \textit{\textbf{local graph}}, used for message passing on inner nodes
    \item the \textit{\textbf{remote graph}}, used for message passing on boundary nodes obtained from other subgraphs along the cut edges. 
\end{itemize}

To reduce the communication volume, \zhuang{the \textbf{\textit{remote graph}} can be further converted to a post-aggregation (post-aggr) graph or a pre-aggregation (pre-aggr) graph.}

% \subsubsection{Traditional Approaches (Pre-Aggregation or Post-Aggregation)} 

\emph{Pre} denotes performing the aggregation operation before communication, while \emph{post} refers to performing the aggregation operation after communication. For instance, consider $S_0$'s perspective of the remote graph $S_1$ shown in Fig.~\ref{fig/method:complicated_graph}. 
In this scenario, the communication volume along the cut edges (dotted line) is 5 nodes' features. By converting the remote graph to either the pre-aggr graph (Fig.~\ref{fig/method:complicated_pre_graph}) or the post-aggr graph (Fig.~\ref{fig/method:complicated_post_graph}, \zhuangppopp{the communication volume can be reduced from 5 node features to 3 node features.}
\zhuang{To the best of our knowledge, most existing solutions choose either the pre-aggregation method~\cite{md2021distgnn} or the post-aggregation method \cite{wan2022bns, wan2023adaptive, mostafa2022sequential, wan2022pipegcn}.}

\subsection{Our Proposal: a Hybrid Aggregation Strategy as MVC problem}\label{sec:hybridaggregation}
% \subsubsection{Our Proposal: a Hybrid Aggregation Strategy}
Both Pre and Post aggregations are suboptimal. So, we propose \textbf{\textit{Pre- and Post- Aggregation}} (Fig.~\ref{fig/method:complicated_optimal_graph}), a simple yet effective method, to achieve a more aggressive reduction in communication volume. With our proposed strategy, the communication volume can be shrunk from 3 nodes to 2 nodes. However, the main challenge is: how to construct pre- and post-aggregation subgraphs. In this subsection, we first construct the pre-post aggregation as solving MVC problem (Sec.~\ref{subsubsec:consructmvc}) and provide a workflow for constructing pre-post aggregation subgraphs (Sec.~\ref{subsubsec:workflowgre}). After constructing the subgraph, we show (Sec.~\ref{subsubsec:comucation})

\subsubsection{Constructing Pre- and Post- Aggregation}\label{subsubsec:consructmvc}
% In This section, we formulate the problem of constructing pre- and post-aggregation subgraphs as solving minimum vertex cover~\cite{{konig1931graphen}}: 

\begin{figure}[t!]
    \centering
    \includegraphics[clip,width=0.48\textwidth]{figures/method/minimum_vertex_cover.pdf}
    \caption{Achieving optimal communication volume via finding minimum vertex cover.}
    \label{fig/method:minimum_vertex_cover}
\end{figure}

Let the remote graph (Fig.~\ref{fig/method:complicated_original_graph}) induce a bipartite graph \(G = (U, V, E)\), where each edge \(e = (u, v) \in E\) represents a data transfer between vertices \(u\) and \(v\). If data were transferred along every edge, a vertex connected to multiple edges might be transmitted repeatedly, leading to redundancy. To eliminate this redundancy, we seek a set of vertices \(C \subseteq U \cup V\) such that every edge is “covered” by at least one vertex in \(C\); mathematically, we require that
\[\footnotesize
\forall (u, v) \in E, \quad u \in C \quad \text{or} \quad v \in C.
\]

This set \(C\) effectively “absorbs” the data transfers for all its incident edges, meaning that transferring the data corresponding to the vertices in \(C\) is sufficient to account for all communications. Our goal is to minimize the communication volume, which is directly proportional to the number of vertices transmitted. Thus, we formulate the problem as
\begin{equation}\footnotesize
\begin{aligned} \label{eq:minimum_vertex_cover}
\min_{C \subseteq U \cup V} |C| \quad \text{subject to} \quad \forall (u,v) \in E, \; u \in C \text{ or } v \in C.
\end{aligned}
\end{equation}

Take Fig.~\ref{fig/method:minimum_vertex_cover}(a) as an example, the goal is to find a vertex set (vertex 2 and 4) that covers all edges while minimizing the number of vertices. Formulation~\ref{eq:minimum_vertex_cover} is exactly the definition of the \textbf{minimum vertex cover (MVC)} problem~\cite{diestel2017graph} on a bipartite graph. So we conclude that \textbf{\textit{finding the optimal communication volume is equivalent to solving the MVC problem on \(G\)}}. The optimal communication volume corresponds to \(|\text{MVC}|\), the minimal number of vertices needed to cover all edges. Also, the MVC problem on bipartite graphs has an optimal solution (by König’s theorem~\cite{konig1931graphen} and Hopcroft–Karp algorithm~\cite{hopcroft1973n}). 

So we can construct the pre- and post-aggregation to achieve optimal communication volume by solving minimum vertex cover. 



\subsubsection{Workflow}\label{subsubsec:workflowgre}
Our proposal categorizes each edge in the remote graph into either the pre-aggr graph or the post-aggr graph \zhuang{at a fine-grained level} (as shown in Algo.~\ref{alg:pre-post-aggregation}).

\zhuang{Initially, we treat the remote graph as a bipartite graph and identify all connected components in this graph. Subsequently, we introduce the minimum vertex cover algorithm to find the nodes that cover all cut edges (line 1-3 in Algo.~\ref{alg:pre-post-aggregation}). In Fig. \ref{fig/method:complicated_original_graph}, nodes $2$ and $4$ form the minimum vertex cover set. Then we traverse all edges in the remote graph (cut edges) (line 4-8 in Algo.~\ref{alg:pre-post-aggregation}). If the source node of the cut edges belongs to the minimum vertex cover (node $4$ and its cut edges). It's better to delay aggregation on these edges until the source node reaches the destination worker to avoid redundant communication (post-aggr). Conversely, when the destination node of cut edges is part of the minimum vertex cover (node $2$ and its corresponding cut edges), aggregation on these edges occurs prior to the transfer of results to the destination worker can reduce redundant communication (pre-aggr). Based on this strategy, a remote graph is transformed into a hybrid of pre-aggr graph and post-aggr graph, as shown in Fig.~\ref{fig/method:complicated_optimal_graph}.}

\input{algorithms/pre_post_aggregation}

Our proposed approach involves the aggregation and communication stages of boundary nodes, including:
\setlength{\leftmargini}{15 pt}
\begin{enumerate}
    \item Perform pre-aggregation on node $5,6$ at $S_1$ to obtain the partial result of node $2$. 
    \item Send node $4$ and the partial result of node $2$ to $S_0$.
    \item Conduct post-aggregation on received node $4$ and the partial result of node $2$ at $S_0$ to get the aggregation result of node $1,2,3$.
\end{enumerate}
% \subsubsection{Performing Pre- and Post-aggregation}



% \subsection{Construting Pre- and Post-aggregation Subgraph is Finding Minimum Vertex Cover}
% \label{sec:permodel_basic}
% \zhuanghpdc{To minimize communication overhead, we formulate the problem as a minimum vertex cover (MVC) in a bipartite graph. This section explains how MVC ensures optimal communication volume.}

% \subsubsection{Minimum Vertex Cover (MVC) in bipartite graphs}
% In a bipartite graph $G = (U, V, E)$, a vertex cover is a subset of vertices $C \subseteq U \cup V$ such that every edge in $E$ has at least one endpoint in $C$. The \textbf{minimum vertex cover} is the smallest such set. König's theorem~\cite{konig1931graphen} establishes that in bipartite graphs, the size of a minimum vertex cover equals the size of a maximum matching, allowing polynomial-time solutions.


% \subsubsection{Achieving Optimal Communication Volume via Minimum Vertex Cover}
% % \begin{figure}[t!]
% %     \centering
% %     \includegraphics[clip,width=0.48\textwidth]{figures/method/minimum_vertex_cover.pdf}
% %     \caption{Achieving optimal communication volume via finding minimum vertex cover.}
% %     \label{fig/method:minimum_vertex_cover}
% % \end{figure}
% Let the remote graph (Fig.~\ref{fig/method:complicated_original_graph}) induce a bipartite graph \(G = (U, V, E)\), where each edge \(e = (u, v) \in E\) represents a data transfer between vertices \(u\) and \(v\). If data were transferred along every edge, a vertex connected to multiple edges might be transmitted repeatedly, leading to redundancy. To eliminate this redundancy, we seek a set of vertices \(C \subseteq U \cup V\) such that every edge is “covered” by at least one vertex in \(C\); mathematically, we require that
% \[\footnotesize
% \forall (u, v) \in E, \quad u \in C \quad \text{or} \quad v \in C.
% \]

% This set \(C\) effectively “absorbs” the data transfers for all its incident edges, meaning that transferring the data corresponding to the vertices in \(C\) is sufficient to account for all communications. Our goal is to minimize the communication volume, which is directly proportional to the number of vertices transmitted. Thus, we formulate the problem as
% \begin{equation}\footnotesize
% \begin{aligned} \label{eq:minimum_vertex_cover}
% \min_{C \subseteq U \cup V} |C| \quad \text{subject to} \quad \forall (u,v) \in E, \; u \in C \text{ or } v \in C.
% \end{aligned}
% \end{equation}

% Take Fig.~\ref{fig/method:minimum_vertex_cover}(a) as an example, the goal is to find a vertex set (vertex 2 and 4) that covers all edges while minimizing the number of vertices. Formulation~\ref{eq:minimum_vertex_cover} is exactly the definition of the \textbf{minimum vertex cover (MVC)} problem~\cite{diestel2017graph} on a bipartite graph. The optimal communication volume corresponds to \(|\text{MVC}|\), the minimal number of vertices needed to cover all edges. Since the MVC problem on bipartite graphs has an optimal solution (by König’s theorem~\cite{konig1931graphen} and Hopcroft–Karp algorithm~\cite{hopcroft1973n}), we conclude that finding the optimal communication volume is equivalent to solving the MVC problem on \(G\). Therefore, an optimal solution for MVC directly yields the optimal communication volume.

% After identifying the vertex set \(C\) of the minimum vertex cover (such as vertex 2 and 4 in Fig.~\ref{fig/method:minimum_vertex_cover}(c)), we construct pre- and post-aggregation graph based on this set, transforming the original edges communication into vertices communication on this set, thereby achieving the optimal communication volume.


\subsection{Communication Performance Model}

\wu{After partitioning the graph and aggregating the nodes, the communication cost required in distributed full-batch GCN training can be estimated. We use ${Comm^{i, j}}$ to represent the communication volume from process $i$ to process $j$. For distributed training with $P$ processes, the communication time $T_{comm}$ is expressed as follows:} 

\begin{equation}\footnotesize
\label{eq:comm_volume}
\begin{aligned}
T_{comm}^{i, j} &= \frac{Comm^{i, j} \times BIT_{fp32}}{BW_{comm}} + L_{comm} \\
T_{comm} &= \max_{i=0}^{P}(\sum_{j=0}^{P}{T_{comm}^{i, j}}) 
\end{aligned}
\end{equation}

\zhuanghpdc{
The upper equation computes the communication time as the sum of the data transfer time, given by \(\frac{V_{comm}^{i, j}}{BW_{comm}}\), and the fixed communication latency \( L_{comm} \).  
Since the communication pattern in distributed full-batch GCN training is highly unbalanced, to account for this imbalance, the lower equation selects the communication time of the process with the longest communication time (serves as the bottleneck) as the global communication time \( T_{comm} \).
}

% In Fig.~\ref{fig/method:complicated_original_graph}, if data is transferred along the edges, the connected vertices may be transmitted multiple times, leading to redundant data transfer. To minimize this redundancy, we need to identify the smallest possible set of vertices that are connected to all edges—ensuring that every data transfer (edge) can be replaced by the transfer of these selected vertices. In other words, by selecting a vertex in this set, we allow it to “absorb” the data transfers for its incident edges. Finding this minimal set of vertices that covers all edges is equivalent to solving the \textbf{minimum vertex cover (MVC)} problem on the bipartite graph induced by the remote graph. 

% The minimum vertex cover $|MVC|$ directly corresponds to the minimal number of aggregation (pre-aggregation and post-aggregation) points required to eliminate redundant data transfers. Any attempt to further reduce communication volume below $|MVC|$ would leave edges uncovered, necessitating additional transmissions. Thus, the communication volume cannot be smaller than the MVC value. We can achieve the lowest communication volume via MVC. 



% \subsection*{Model Setup}

% 1. \textbf{Bipartite Graph Representation:}  
%    Let \( G = (U, V, E) \) represent the communication graph, where:
%    \begin{itemize}
%        \item \( U \): Set of source nodes (e.g., compute nodes generating raw data).
%        \item \( V \): Set of destination nodes (e.g., nodes requiring aggregated results).
%        \item \( E \): Edges with weights denoting raw data volume between nodes.
%    \end{itemize}

% 2. \textbf{Aggregation Strategies:}
%    \begin{itemize}
%        \item \textbf{Pre-aggregation (at \( U \))}: A source node \( u_i \in U \) aggregates data locally before transmission, reducing outgoing edges to a single unit.
%        \item \textbf{Post-aggregation (at \( V \))}: A destination node \( v_j \in V \) aggregates incoming data, reducing incoming edges to a single unit.
%    \end{itemize}

% 3. \textbf{Objective:}  
%    Minimize the total communication volume by selecting a subset of nodes \( C \subseteq U \cup V \) to perform aggregation, such that:
%    \begin{itemize}
%        \item Every edge \( (u_i, v_j) \in E \) is "covered" by at least one node in \( C \): either \( u_i \) (pre-aggregation) or \( v_j \) (post-aggregation).
%        \item Total communication volume equals the size of \( C \) (each aggregated node contributes 1 unit) plus the number of edges \textit{not} covered by \( C \) (each requiring full transmission).
%    \end{itemize}

% \subsection*{Key Steps}

% 1. \textbf{Equivalence to Minimum Vertex Cover (MVC):}  
%    The problem reduces to finding the smallest \( C \) (MVC) that covers all edges in \( E \). By König’s theorem, in bipartite graphs:
%    \[
%    |\text{MVC}| = |\text{Maximum Matching}|
%    \]
%    This ensures \( |C| \) is minimal.

% 2. \textbf{Lower Bound on Communication Volume:}  
%    \begin{itemize}
%        \item If an edge \( (u_i, v_j) \) is \textbf{not covered} by \( C \), the raw data must be transmitted directly, incurring its full weight (e.g., 1 unit per edge).
%        \item If an edge is \textbf{covered} by \( C \), aggregation reduces its contribution to 1 unit (either at \( u_i \) or \( v_j \)).
%        \item Total communication volume \( \text{Comm}(C) \) satisfies:
%          \[
%          \text{Comm}(C) \geq |C| + \text{(Uncovered edges)}
%          \]
%          Since all edges must be covered by \( C \), \textbf{uncovered edges = 0}, hence:
%          \[
%          \text{Comm}(C) \geq |C|
%          \]
%    \end{itemize}
%    The minimal \( |C| \) (i.e., MVC) thus provides the theoretical lower bound for communication volume.

% 3. \textbf{Optimality via König’s Theorem:}  
%    Suppose there exists a strategy with communication volume \( \text{Comm} < |\text{MVC}| \). This would imply:
%    \begin{itemize}
%        \item Fewer aggregation points than \( |\text{MVC}| \), violating the definition of MVC (smallest set covering all edges).
%        \item At least one edge remains uncovered, forcing its full transmission, which contradicts \( \text{Comm} < |\text{MVC}| \).
%    \end{itemize}


% Let the communication graph be modeled as a bipartite graph \( G = (U, V, E) \), where \( U \) and \( V \) represent source and destination nodes, respectively, and edges \( E \) denote communication links. A **minimum vertex cover (MVC)** \( C \subseteq U \cup V \) is the smallest subset of nodes covering all edges.  

% 1. **Aggregation Strategy:**  
%    - A node \( u_i \in C \cap U \) performs *pre-aggregation*, reducing outgoing data.  
%    - A node \( v_j \in C \cap V \) performs *post-aggregation*, reducing incoming data.  

% 2. **Equivalence to MVC:**  
%    By König’s theorem \cite{Konig1931}, \( |\text{MVC}| = |\text{Maximum Matching}| \). Thus, \( |C| \) is minimal.  

% 3. **Lower Bound Derivation:**  
%    - Each node in \( C \) contributes 1 unit of communication (aggregated data).  
%    - If \( \text{Comm} < |C| \), there exists an edge \((u_i, v_j)\) not covered by \( C \), requiring raw data transfer (contradicting minimality).  

% Hence, the communication volume cannot be smaller than \( |\text{MVC}| \).  

% **Formal Proof:**  
% Assume for contradiction that \( \text{Comm}^* < |\text{MVC}| \). By König’s theorem, \( |\text{MVC}| \) equals the maximum matching size. If \( \text{Comm}^* < |\text{MVC}| \), fewer than \( |\text{MVC}| \) nodes cover all edges, violating MVC’s minimality. Thus, at least one edge remains uncovered, forcing full data transmission and contradicting \( \text{Comm}^* \).  

% ---  
% This proof aligns with König’s theorem, ensuring the MVC-based strategy achieves the theoretical lower bound for communication in distributed systems.  

% ```latex
% % In LaTeX, ensure proper theorem citations and formatting:
% \cite{Konig1931} % Reference entry required in bibliography
% ```


% Once these vertices are identified, we further optimize communication:  
% a) \emph{Post-aggregation}: If a selected vertex belongs to the source graph, sending it to the destination graph eliminates the communication (edges) where it acts as a source node, reducing incoming data.
% b) \emph{Pre-aggregation}: If a selected vertex belongs to the destination graph, we perform pre-aggregation. By sending the aggregation result (i.e., the vertex itself) to the destination graph, we remove all communications (edges) where it serves as a destination node, reducing incoming data. Since the MVC problem on the bipartite graph can be solved in polynomial time, we can achieve the lowest communication volume in polynomial time.

% By selecting the minimum vertex cover of the communication graph (as shown in Fig.~\ref{fig/method:complicated_optimal_graph}), we ensure that every data transfer is "covered"—meaning that for each required transfer, at least one endpoint processes the data locally. This strategy reduces overall communication overhead because a single node can handle multiple transfers, eliminating redundant data movement. In summary, solving the bipartite minimum vertex cover problem directly yields the optimal set of nodes needed to minimize communication.



% A bipartite graph \( G = (U, V, E) \) partitions vertices into two disjoint sets \( U \) and \( V \) (vertices in Fig.~\ref{fig/method:complicated_graph}), where edges \( E \) (edges in Fig.~\ref{fig/method:complicated_graph}) connect vertices only across these sets. A \textbf{minimum vertex cover} is the smallest subset of vertices \( C \subseteq U \cup V \) such that every edge in \( E \) is incident to at least one vertex in \( C \). By König's theorem, in bipartite graphs, MVC can be solved in polynomial time.

% \subsubsection{Obtain optimal communication volume by Minimum Vertex Cover (MVC)} Consider the remote graph in Fig.~\ref{fig/method:complicated_graph} as a bipartite graph, where set $S_0$ represents dst vertices, $S_1$ represents src vertices, edges from $S_1$ to $S_0$ represent communication. The goal is to cover all necessary communications (edges) while minimizing the total transferred data. 

% To minimize the total communication volume, each data transfer (each edge) is "covered" by at least one endpoint where the data can be processed locally. If a node is selected as part of our solution (i.e., it belongs to the vertex cover), then all edges incident to it do not incur full communication cost. Thus, selecting a minimum set of nodes that cover all edges is equivalent to minimizing the total communication volume.


% \zhuanghpdc{During communication based on the remote graph representation, for each edge, we only need to transfer either its corresponding source node or destination node. Since different edges may share the same source or destination nodes, multiple edges can potentially be represented by transferring a single vertex that corresponds to all of them. Therefore, to achieve optimal communication volume, our objective is to identify the minimal set of vertices in the remote graph that can represent all edges. In other words, we aim to find the minimum vertex set that covers (touches) all edges. This problem definition aligns with the classical minimum vertex cover problem in graph theory. Consequently, we can transform the problem of finding optimal communication volume into solving the minimum vertex cover problem on the remote graph. Since the remote graph can be modeled as a bipartite graph, the minimum vertex cover problem on bipartite graphs can be solved optimally in polynomial time using the Hopcroft-Karp algorithm~\cite{hopcroft1973n} through its connection to maximum matching. This implies that given a graph partitioning result, we can find the optimal communication volume for GNN computations in polynomial time.}



% \wu{
% The upper equation calculates the communication time by accumulating the data transfer time $\frac{V_{comm}^{i, j}}{BW_{comm}}$ and the fixed communication latency $L_{comm}$. 
% Since communication in a distributed full-batch GCN training is highly unbalanced, some processes are bounded by bandwidth, while others may be bottlenecked by latency.
% The lower equation identifies the process with the highest communication time, which serves as the overall bottleneck and dictates the final communication time \( T_{comm} \).
% }



% The inner summation accumulate $\frac{Data^j_i}{BW_{comm}}$ and $L_{comm}$, as communication in a distributed GCN is highly unbalanced and may be constrained by either a throughput bottleneck or a latency bottleneck. 
% The sum over j aggregates the total communication time for process i.
% The outer max function determines the final communication time by identifying the process with the highest total time, which serves as the overall bottleneck in the framework's communication.


% After partitioning the graph, the number of nodes transferred from one process to another is denoted by \( N_{\text{transfer}} \), the length of the embedding (feature vector) is \( L_{\text{feat}} \), the number of GCN layers is \( N_{\text{layer}} \), the total number of processes is \( P \), the number of bits per element is \( Bit_{\text{fp32}} \).  Each GCN layer requires one collective communication. Without the use of quantization, the total communication volume (in bits) is given by:
% \begin{equation}\tiny
% \label{eq:comm_volume}
% V_{\text{comm}} = P \cdot (P - 1) \cdot N_{\text{layer}} \cdot N_{\text{transfer}} \cdot L_{\text{feat}} \cdot Bit_{\text{fp32}}
% \end{equation}

% By using the pre-post aggregation method to transform the remote graph, we have 
% \begin{equation}\tiny
% N_{\text{transfer}} \leq \min(\# src\_nodes\_of\_cut\_edges, \# dst\_nodes\_of\_cut\_edges)
% \end{equation}
% Therefore, compared to pre-aggregation and post-aggregation, the proposed hybrid approach reduces the total communication volume.

% \subsubsection{Quantization of communication to Int2}

\begin{comment}
\subsection{\zhuanghpdc{Efficient int2 quantization communication}}

\label{subsec:quantized_communication}

In a distributed GNNs training system, boundary node feature vectors are transferred across subgraphs in FP32. To reduce communication volume, \zhuanghpdc{the previous work~\cite{wan2022bns} propose an adaptive quantization communication for GPU. The procedure is illustrated in Fig.~\ref{xxx}. With further analysis, we found that there are several issues: (1) Their method requires a centralized bit-width master assigner that determines the bit-width of communication for each worker by solving a bi-objective optimization problem. This will limit the framework's scalability. (2) Compared with general GPU clusters, CPU supercomputers have worse absolute performance per node than GPUs (especially considering that we assign an MPI process to a numa node), but CPU supercomputers generally have similar collective communication performance (especially there are vendor-optimized communication libraries for scalable interconnection network on CPU supercomputers, such as Fujitsu MPI and TofuD 6d torus interconnection on Fugaku). Therefore, the overhead of quantization and dequantization on CPUs is much larger than on GPU clusters. (3) TODO: Splitting the original communication into two will incur two synchronization overheads. In addition, considering that each row of quantized parameters contains only two bfloat16 numbers, the communication of parameters will shift to latency-bound when we scale to a large number of workers. To solve the above potential issue of adaptive quantization communication in \cite{wan2022bns}, we propose an efficient and decentralized pure int2 quantization communication scheme. To address the potential accuracy loss problem, we innovatively introduce label propagation to reduce the noise caused by int2 quantization. }

\subsubsection{An efficient int2 quantization communication scheme}
\zhuanghpdc{Our proposed efficient and decentralized pure int2 quantization communication scheme is shown in Fig.~\ref{xxx}. In our proposed scheme, each worker compresses the message to int2 and recovers the message back to fp32 without any synchronization or communication with a centralized master. There are several key optimizations in our proposed scheme:}

\zhuanghpdc{(1) Fusion of computing quantization parameters kernel and quantization kernel. In the computing quantization parameter kernel, we scan the entire message matrix in fp32 to get each row's parameters \textit{zero-point} and \textit{scale}. After that, we scan the whole message matrix in fp32 again to quantize the data. To reduce the redundant memory access, in the fused kernel, we first get the 4 rows of data in the original message matrix and calculate the quantization parameter for these 4 rows. After that, we immediately get the data from the L1 cache and quantize the data using the parameters just calculated.}

\zhuanghpdc{(2) Latency reduction in quantization kernel. In the original quantization process, there is a division operation that has long latency (e.g. 98 cycles on Futjisu A64FX~\cite{xxx}). To shorten instruction dependency chains and improve instruction throughput, we replace this division operation with reciprocal estimate and multiplication operations, which have shorter latency and higher throughput. In addition, we also remove the random number operation in quantization to further improve the performance of the quantization kernel.}

\zhuanghpdc{(3) Vectorization for quantization and dequantization kernel on different CPUs. }

\zhuanghpdc{(4) TODO: Message packaging. }

\subsubsection{Accuracy recovery by label propagation.}

% we quantize the features of all boundary nodes to Int2 before communication and dequantize them to FP32 after communication. To reduce the overhead of quantization, we optimize the quant/dequant kernel by using CPU SIMD instructions and improving data layout.

To reduce the potential model accuracy degradation caused by Int2 communication, we introduce label propagation in our framework.
\zhuanghpdc{To the best of our knowledge, this work is the first to employ pure Int2 communication and apply label propagation to recover model accuracy. In label propagation, before training begins, we randomly select a batch of nodes (at a fixed sampling rate) from those with training labels and perform an embedding operation on their labels. We then add the label embeddings to the initial feature vectors of these selected nodes. The procedure is shown in Fig.~\ref{fig/method:overview_procedure} \circled{3}. This step allows the labels to propagate along with the feature vectors during neighbor aggregation. The remaining unselected nodes with training labels are used to update the model.}

\textbf{Lemma 1.} \zhuanghpdc{With our quantization scheme, the model convergence rate is still maintained $O(\frac{1}{T})$ for $T$ epochs with a gradient variance bound $K$.}

\textbf{Lemma 2.} \zhuanghpdc{For each GNN layer {\small $l \in \{1,...,L\}$}, we reduce the adaptive quantization Theorem in~\cite{wan2023adaptive} to confine the bit-width $B$ to 2 for the scaling factor term. We have the gradient variance upper bound $K^l$ in layer $l$:}
\begin{equation}\tiny \label{eq:var}
\begin{split}
    K^l =&  \sum_i^{|V|}(\sum_{j=i}^{N_R(i)} \sum_{u=i}^{N_R(i)} \alpha_{ji}^2 \alpha_{ui}^2  \frac{D_{j}^{l-1}D_{u}^{l}(S_{j_2}^{l-1}S_{u_2}^{l})^2}{6} \\ 
    & + M^2\cdot \sum_{j=i}^{N_R(i)} \frac{\alpha_{ji}^2 D_j^l(S_{j_2})^2}{6} + N^2 \cdot \sum_{j=i}^{N_R(i)}\alpha_{ji}^2 \frac{D_j^{l-1}(S_{j_2}^{l-1})^2}{6})
\end{split}
\end{equation}

\zhuanghpdc{where the $|V|$ is the number of nodes, $N_R(i)$ is the remote neighbors of node $i$, $j$ and $u$ both represent each neighbors of node $i$, $\alpha_{ji}$ and $\alpha_{ui}$ is the coefficient brought from $i$'s remote neighbors $j$ and $u$, respectively. $D_j$ and $D_u$ are the dimensions of the features of $i$'s remote neighbors $j$ and $u$. $j_b$ and $u_b$ is the bit width assigned to the features sent from $i$'s remote neighbors $j$ and $u$. $S_{j_b}$ and $S_{u_2}$ is the scaling factor that maps the original FP32 to the quantized int2 {\small$Scale = \{max(h)-min(h)\}/{(2^{j_2}-1})$}.}

\textbf{Proposition 1.} \zhuanghpdc{By integrating label propagation into feature propagation, the connectivity between nodes with the same label is enhanced, which leads to a lower variance upper bound $K^l$ in Eqn.~\ref{eq:var}, thereby decreasing the accuracy loss caused by quantization.}


% Label propagation increases the influence among nodes with the same label~\cite{shi2020masked}, thereby reducing the noise introduced by remote neighbors' Int2 feature vector during neighbor aggregation.

% To the best of our knowledge, this work is the first to employ pure Int2 communication and apply label propagation to recover model accuracy. In label propagation, before training begins, we randomly select a batch of nodes (at a fixed sampling rate) from those with training labels and perform an embedding operation on their labels. We then add the label embeddings to the initial feature vectors of these selected nodes. The procedure is shown in Fig.~\ref{fig/method:overview_procedure} \circled{3}. This step allows the labels to propagate along with the feature vectors during neighbor aggregation. The remaining unselected nodes with training labels are used to update the model. Label propagation increases the influence among nodes with the same label~\cite{shi2020masked}, thereby reducing the noise introduced by remote neighbors' Int2 feature vector during neighbor aggregation.

% \begin{figure}[t]
%     \centering
%     \subfigure[$S_0$'s remote graph. 
%     The transferred data volume is 5.
%     ]{
%         \begin{minipage}[b]{0.2\textwidth}
%             \includegraphics[width=1\textwidth]{figures/method/complicated_original_graph.pdf}
%         \end{minipage}
%         \label{fig/method:complicated_original_graph}
%     } \hspace{2mm}
%     \subfigure[Convert to Pre-aggr graph. 
%     The transferred data volume is 3.~\cite{md2021distgnn}
%     ]{
%         \begin{minipage}[b]{0.2\textwidth}
%         \includegraphics[width=1\textwidth]{figures/method/complicated_pre_graph_v1.pdf}
%         \end{minipage}
%     \label{fig/method:complicated_pre_graph}
%     } 
%     \\
%     \subfigure[Convert to Post-aggr graph. 
%     The transferred data volume is 3.~\cite{wan2022bns, wan2023adaptive, mostafa2022sequential, wan2022pipegcn}
%     ]{
%         \begin{minipage}[b]{0.2\textwidth}
%             \includegraphics[width=1\textwidth]{figures/method/complicated_post_graph_v1.pdf}
%         \end{minipage}
%         \label{fig/method:complicated_post_graph}
%     } \hspace{2mm}
%     \subfigure[Convert to the \zhuang{hybrid} of post-aggr and pre-aggr graph. 
%     %The transferred data volume is 2 (Optimal).
%     ]{
%         \begin{minipage}[b]{0.2\textwidth}
%         \includegraphics[width=1\textwidth]{figures/method/complicated_optimal_graph_v1.pdf}
%         \end{minipage}
%     \label{fig/method:complicated_optimal_graph}
%     } 
%     \caption{Different strategies to reconstruct a remote graph.}
%     \label{fig/method:complicated_graph}
% \end{figure}
In the typical distributed GNNs training system, boundary node feature vectors are transferred across subgraphs in FP32 (32-bits). Wan et al.~\cite{wan2023adaptive} demonstrates that it's possible to transfer these feature vectors in int8, int4, and even int2, reducing communication overhead, without compromising model convergence and even achieving higher model accuracy. To strike a balance between performance and model accuracy, they introduce a sophisticated adaptive integer bit width assignment algorithm for determining the feature vector bit width of each boundary node. Nevertheless, their experiments show that even with a simple and low-overhead sampling algorithm, this balance can still be achieved. Therefore, we propose a straightforward sampling algorithm for the bit width determination of each boundary node based on a predefined probability:
\begin{equation}\footnotesize 
Bits = \left\{
\label{eq:bits_assignment}
\begin{aligned}
& int8, \hspace{2pt} Prob(int8)
\\
& int4, \hspace{2pt} Prob(int4)
\\
& int2, \hspace{2pt} 1-Prob(int8)-Prob(int4)
\end{aligned}
\right.
\end{equation} 
% In this approach, we quantize the feature vectors of all boundary nodes using our quantization kernel based on the bit width determination result before communication and then dequantize them to FP32 with our dequantization kernel after communication.
During further experiments, we've discovered that even when fixing the bit width of each boundary node to int2 (meaning all boundary node feature vectors are quantized to int2), we can still maintain the model's convergence rate and accuracy. As a result, we propose a quantization communication method based on this finding. In this approach, we quantize the feature vectors of all boundary nodes to int2 using our quantization kernel before communication, and then dequantize them to FP32 with our dequantization kernel after communication. 
\end{comment}


%\subsection{Summary of the end-to-end flow of our proposed framework}
%\label{subsec:procedure}

%\end{enumerate}

% In our proposed system, the (c) \emph{Aggregation operator} manages to solve the problem of irregular memory access and load imbalance for the performance bottleneck aggregation operators on different CPUs, which serves as the performance foundation for the entire system. 
% The (a) \emph{Graph partitioner}, (b) \emph{Subgraph constructor}, (c) \emph{Random integer bits assigner}, and (e) \emph{Communicator} collaborate to reduce the communication volume and alleviate the pressure on system scalability posed by the communication overhead.

% \subsection{Random integer bits assigner}
% Each boundary node's feature can be quantized into int8, int4, or int2. Quantizing all features into int8 provides more benefits in terms of model accuracy but sacrifices performance. Conversely, quantizing all features into int2 yields more performance benefits but less improvement in accuracy. Therefore, a strategy to determine the bit width of each feature is necessary. Different from solving a complex bi-object optimization problem in \cite{wan2023adaptive}, we propose a random integer bit assigner, as shown in Equation \ref{eq:bits_assignment}. This random assigner sets the probability of each bit width before training, and the bit width of each feature will be updated randomly and periodically based on the preset probability. The preset probability can be adjusted based on the practical demand.

% \subsection{Efficient quantizer and dequantizer on CPUs}
% To reduce the overhead caused by quantization and dequantization, we implement efficient quantizer and dequantizer based on SIMD instructions for both x86 CPUs and ARM CPUs. We employ stochastic integer quantization methods as shown in Equation \ref{eq:quantization} and \ref{eq:dequantization}.



% \subsection{Communicator}
% The communicator is used to transfer two types of data: (1) the quantization parameters employed for dequantization on other machines, and (2) the boundary nodes' feature which has been pre-aggregated and quantized using the bit widths assigned by the random integer bits assigner. The communicator utilizes the MPI\_Alltoallv primitives optimized for supercomputers for data transfer. To further decrease the communication overhead, when transferring the extensive amount of boundary nodes' features, the communicator switches to an asynchronous mode. In this mode, the communication of boundary nodes' features is overlapped with the aggregation on the local graph since these are two independent operations.


==> 3-implementation.tex <==
\label{sec:implementation}

Our proposed system is built on top of PyTorch Geometric (PyG) \cite{fey2019pyg}. Currently, PyG lacks support for distributed full-batch GNNs training. Consequently, we implement the entire process including graph partitioning, data assignment, and subgraph construction by ourselves. 

For graph partitioning, We use ParMetis \cite{karypis1997parmetis}\todo{Cite}, a widely used mini-cut graph partitioning algorithm employed in traditional graph processing systems and GCNs. To ensure a balanced distribution of training samples and prevent load imbalances among different workers, we assign multiple node weights based on factors like the in-degree of nodes and training masks when configuring ParMetis.

It's worth noting that the quantization and dequantization kernel in PyTorch is extremely slow on CPU side. Therefore, to mitigate the overhead incurred by quantization and dequantization, we developed efficient quantization and dequantization kernels based on SIMD instructions for both x86 CPUs and ARM CPUs. We employ stochastic integer quantization methods illustrated in Equation \ref{eq:quantization} and \ref{eq:dequantization}.

==> 4-proof.tex <==
\label{sec:proof}

\input{tables/datasets_models}


% \subsection{Impact of \emph{pre- and post-aggregation} on model training convergence}
% The proposed \emph{pre- and post-aggregation} method only divides the entire aggregation operators into several smaller aggregation operators and changes the order of these independent operators. The combination of them still can be treated as the original entire aggregation operators. The graph structure information and the training procedure haven't been changed. Therefore, this method doesn't exert a negative effect on model training convergence. 

% \subsection{Impact of \emph{random bit integer quantization} on model training convergence}
We show the impact of our quantization scheme on the model convergence variance bound while maintaining the convergence rate of $O(\frac{1}{T})$ for $T$ epochs. The proofs of the lemma are provided in the Supp. material. In the method of \emph{quantization communication}, the boundary nodes' features are compressed from FP32 to int2 through the stochastic integer quantization \cite{chen2021actnn}, which incurs the loss of numerical precision. 
%The quantization method we apply is similar to the method used in \cite{wan2023adaptive}. Building upon their work, we improve the strategy for selecting bit widths of each feature vectors.
Since we use SGD as an optimizer, the full-batch GNNs training can be formulated as the following non-convex minimization problem, the target is to find the global minimum.
\begin{equation}\tiny 
\label{eq:dequantization}
\operatorname*{argmin}_{W_t \in \mathbb{R}^D} \mathbb{E}[\mathcal L(W_t)] = \frac{1}{n}\sum_{i=1}^n \mathcal L(W_t, X_i), W_{t+1} = W_t - \eta \nabla \widetilde {\mathcal L}(W_t)
\end{equation}

while $W_t$ refers to the weight parameters of the model at the epoch t, $D$ is the dimension of the $W_t$, $\mathcal L(W_t, X_i)$ is the loss on training sample $X_i$ i.e. the node in the graph, $n$ is the number of training samples, $\eta$ is the learning rate, $\nabla \widetilde {\mathcal L}(W_t)$ is the approximate gradient in our quantization methods. As we discussed before, the variance in $\nabla \widetilde {\mathcal L}(W_t)$ is only incurred by the stochastic quantization methods. 

\textbf{Lemma 1.} With the GNNs model, given a global minimum of loss $\mathcal L(W^*)$, we make the following assumptions:

(1) the gradient $\nabla \widetilde {\mathcal L}(W_t)$ are $\rho$-Lipschitz continuous, (2) the approximate gradient is unbiased, {\small $\mathbb{E}[\nabla \widetilde {\mathcal L}(W_t)] = \nabla {\mathcal L}(W_t)$}, (3) the variance of the approximate gradient is bounded, 
{\small$Var[\lVert \nabla \widetilde {\mathcal L} (W_t) - \nabla \mathcal L(W_t) \rVert_2] = \mathbb{E}[\lVert \delta_t \rVert_2] \leq K$}, $K$ is a constant and $K > 0$.

Then select any t in epoch{\small \{1,...,T\}}, we have 
\begin{equation}\tiny
\mathbb{E}[\lVert \nabla \widetilde {\mathcal L} (W_t) \rVert_2^2] \leq \frac{2 ({\mathcal L} (W_1) - {\mathcal L} (W^*))}{T(2\eta-\rho\eta^2)} + \frac{\eta\rho}{2-\eta\rho} \cdot K^2 
\end{equation}

The first term of the right side will go to $0$ while {\small$T \rightarrow \infty$}. This means under the quantization scheme we maintain {\small$O (\frac{1}{T})$} converge rate, and consequently the the model will converge to the neighborhood of a stationary point, the radius of the neighborhood is determined by the gradient variance $K$. Here we introduce Lemma 2 which is a reduced version of the adaptive quantization Theorem in~\cite{wan2023adaptive} to determine the upper bound of gradient variance $K$ when we use a fixed bit width for all layers:

\textbf{Lemma 2.} Given a distributed graph {\small$G(V, E)$}, suppose:
In each layer {\small$l \in \{1,...,L\}$} of the GNNs and each node $v$ in the graph, for the aggregated features {\small $Z_i^{l-1} = %AGGREGATE(h_j^{l-1} \mid j \in N(i)) = 
\sum_{j = i}^{N(i)}\alpha_{ij} \cdot h_j$ }and the aggregated gradients{\small $\frac{\partial {\mathcal L}}{\partial Z_i^{l}} = 
% AGGREGATE(\frac{\partial {\mathcal L}}{\partial Z_j^{l}} \mid j \in N(i)) = 
\sum_{j = i}^{N(i)}\alpha_{ij} \cdot \frac{\partial {\mathcal L}}{\partial Z_j^{l}}$, the $L_2$ 
}norm of the expectation of the aggregated features and the aggregated gradients are bounded by a constant M and N, respectively.

Then for each GNN layer {\small $l \in \{1,...,L\}$}, we reduce the adaptive quantization Theorem in~\cite{wan2023adaptive} to confine the bit-width $B$ to 2 for the scaling factor term. We have the gradient variance upper bound $K^l$ in layer $l$:
\begin{equation}\tiny \label{eq:var}
\begin{split}
    K^l =&  \sum_i^{|V|}(\sum_{j=i}^{N_R(i)} \sum_{u=i}^{N_R(i)} \alpha_{ji}^2 \alpha_{ui}^2  \frac{D_{j}^{l-1}D_{u}^{l}(S_{j_2}^{l-1}S_{u_2}^{l})^2}{6} \\ 
    & + M^2\cdot \sum_{j=i}^{N_R(i)} \frac{\alpha_{ji}^2 D_j^l(S_{j_2})^2}{6} + N^2 \cdot \sum_{j=i}^{N_R(i)}\alpha_{ji}^2 \frac{D_j^{l-1}(S_{j_2}^{l-1})^2}{6})
\end{split}
\end{equation}

where the $|V|$ is the number of nodes, $N_R(i)$ is the remote neighbors of node $i$, $j$ and $u$ both represent each neighbors of node $i$, $\alpha_{ji}$ and $\alpha_{ui}$ is the coefficient brought from $i$'s remote neighbors $j$ and $u$, respectively. $D_j$ and $D_u$ are the dimensions of the features of $i$'s remote neighbors $j$ and $u$. $j_b$ and $u_b$ is the bit width assigned to the features sent from $i$'s remote neighbors $j$ and $u$. $S_{j_b}$ and $S_{u_2}$ is the scaling factor that maps the original FP32 to the quantized int2 {\small$Scale = \{max(h)-min(h)\}/{(2^{j_2}-1})$}. 
\zhuangppopp{According to Lemma 2, the gradient variance is partly affected by $S_{j_2}$, related to the target quantization bit width of each node's features, and $\alpha_{ji}$ and $\alpha_{ui}$, being the coefficient brought from $i$'s remote neighbors $j$ and $u$, respectively. We use a fixed bit width 2 for quantization. }

\zhuangppopp{\textbf{Lemma 3.} With the GCNs model, by embedding the label into the vector space of the feature, label propagation and feature propagation are approximately unified into message passing operations in GCNs. That is to say, we have:}
\begin{equation}\tiny 
\begin{split}
    H^{(l+1)} = AH^{(l)}W^{(l)} = A^{l}(X+Y_{embed})(W^{(0)}W^{(1)} \cdots W^{(l)}) \\
    = A^{l}X(W^{(0)}W^{(1)} \cdots W^{(l)}) +  A^{l}Y_{embed}(W^{(0)}W^{(1)} \cdots W^{(l)})
\end{split}
\end{equation}

\zhuangppopp{where $H^{(l)}$ is the embedding after GCN layer $l$, $A$ is the adjacent matrix, $W^{l}$ is the weight matrix in GCN layer $l$, $X$ is the initial feature vectors, $Y_{embed}$ is the embedding from label, while $Y_{embed} = YW_{embed}$. 
According to Lemma 3, adding embedded labels into features can be treated as a type of label propagation. Based on \cite{shi2020masked}, integrating label propagation into feature propagation can enhance the connectivity between nodes with the same label. This increased connectivity allows nodes with the same label to cluster during message passing, enabling the classifier to more precisely separate nodes with different labels. This enhances the model's tolerance to precision loss. Consequently, most of $\alpha_{ji}$ and $\alpha_{ui}$ in Eqn.~\ref{eq:var}, which represent the connectivity to remote neighbors, are reduced. This reduction leads to a lower variance $K^l$ in Eqn.~\ref{eq:var}, thereby decreasing the loss caused by quantization.} 
% According to Lemma 2, the gradient variance is partly affected by $S_{j_2}$ that is related to the target quantization bit width of each node's features. Instead of tackling the complex bi-objective optimization problem as suggested by~\cite{wan2023adaptive}, we build on the empirical observation that int2 quantization communication has no notable negative impact on accuracy, and use a fixed bit width for features. % based on the preset probability. %, which can adjust the value of $S_{j_2}$ to strike a balance between the model convergence and performance. It is noteworthy that our randomized method introduces some randomness which enhances the generalization ability of the model. 


% For the naive method which quantizes all features in a single bit width, \cite{wan2023adaptive} has proved that the convergence rate is $O(T^{-1})$ under the standard assumptions that are usually used for model convergence analysis.

% To enhance performance while minimizing gradient variance in the weight matrix during model training, it's vital to carefully select the quantized bit width for each feature. Instead of tackling a complex bi-objective optimization problem, we adopt a randomized approach to assign bit widths to features. To strike a balance between performance and gradient variance, we dynamically adjust the probability of each bit through auto-tuning. This allows for more aggressive bit width selection, ultimately leading to the discovery that using pure int2 (with a 100\% probability) is a feasible strategy for achieving model convergence.


==> algorithms/optimized_index_add.tex <==
\SetKw{KwBy}{by}

\newcommand*{\AddNote}[4]{%
    \begin{tikzpicture}[overlay, remember picture]
        \draw [decoration={brace,amplitude=0.5em},decorate,thick,red]
            ($(#3)!(#1.north)!($(#3)-(0,1)$)$) --  
            ($(#3)!(#2.south)!($(#3)-(0,1)$)$)
                node [align=center, text width=2.5cm, pos=0.5, anchor=west] {#4};
    \end{tikzpicture}
}%

\begin{algorithm}[t]
    %\begin{minipage}{0.99\linewidth}
      \small
\caption{Optimized implementation of index\_add operators.}
\label{alg:optimized_index_add}   

\KwIn{array $src$, array $idx$, size of array $idx$ $len\_idx$, length of vertices feature $len\_vec$, length of register kernel $N$}
\KwOut{array $dst$} 
    $dict$ {$\gets$} generate\_dict($idx$, $src$) 

    % \For{$i=0$ \KwTo $len\_idx$} {
    %     $dict[i].first$ {$\gets$} $idx[i]$ \Comment{set idx as keys}

    %     $dict[I].second$ {$\gets$} $\&(src[i][0])$ \Comment{set ptr to src as values}
    
    % }

    $sorted\_dict$ {$\gets$} parallel\_sort($dict$) \Comment{sort $dict$ based on $idx$}

    $flops$ {$\gets$} count\_works($sorted\_dict$) \Comment{count works from each row of $dst$}

    $r\_begin$, $r\_end$, $c\_begin$, $c\_end$ {$\gets$} divide\_work($flops$, $len\_vec$, $n\_th$, $tid$) \Comment{divide work for 2d dynamic parallelism}

        {\color{blue}\#pragma omp parallel} \Comment{launch multiple threads}
    
        \For(\Comment{parallel on $dst$'s rows}){$i=r\_begin$ \KwTo $r\_end$ } { 

            $idxr\_begin$ {$\gets$} $accu\_num\_works[i]$
    
            $idxr\_end$ {$\gets$} $accu\_num\_works[i+1]$
    
            \For(\Comment{parallel on $dst$'s cols}){$j=c\_begin$ \KwTo $c\_end$} { 
                \tikzmark{top}
                \For(\tikzmark{right}){$k=idxr\_begin$ \KwTo $idxr\_end$} { 
    
                    % register\_kernel($dst$, $src$, $idx$, $i$, $j$, $k$) \Comment{invoke register kernel}
% \Comment{can replace with reg kernel}
                
                    dst[i][j] += src[k][j]  
                    \tikzmark{bottom}
                    \AddNote{top}{bottom}{right}{replace with register kernel}
                } 
            
            }

        } 
    
\end{algorithm}

==> algorithms/original_index_add.tex <==
\begin{algorithm}[t]
    %\begin{minipage}{0.99\linewidth}
      \small
\caption{Original implementation of index\_add operators.}
\label{alg:original_index_add}   

\KwIn{array $src$, array $idx$, size of array $idx$ $len\_idx$, length of vertices feature $len\_vec$}
\KwOut{array $dst$} 

    \For{$i=0$ \KwTo $len\_idx-1$} {
    
        $row\_dst$ {$\gets$} $idx[i]$ \Comment{get row idx of $dst$}
        
        {\color{blue}\#pragma omp parallel for} \Comment{launch multiple threads} 
        
        \For(\Comment{parallel on $dst$'s cols}){$j=0$ \KwTo $len\_vec$} {
            $dst[row\_dst][j]$ += $src[i][j]$ \Comment{accumulate $src$ to $dst$}
        }
        
    }

\end{algorithm}

==> junk.tex <==
**Q**: Is such system better than GPU clusters?
**A**: We compared our system with a SoTA GPU system on a dataset in section 5.8. For GPUs of the same generation as the CPUs on the Fugaku supercomputer, we believe our system performs better than the GPU-based system as Fugaku has powerful interconnection.


**Q**: In Figure 9, the "other time" can be reduced by SuperGCN.
**A**: "Other time" includes some overhead of memory buffer. Communication optimization reduces the communication buffer size, thus decreasing the "other time" slightly.

**Q**: Why can α_ji and α_ui be reduced?
**A**: After applying label propagation, the connectivity between the central node and a small subset of neighbors with the same label is strengthened. In contrast, the connectivity with most neighbors that have different labels, including most remote neighbors, weakens. Consequently, most coefficients α_ji and α_ui, which represent the connectivity, decrease.


Because node-level operators serve as a basis for achieving large-scale and communication optimization is more important, we did not design too many experiments about the node-level operators.


For GAT, the training procedure is different since we need to calculate and transfer the learnable weight of neighbors, which exposes different optimization opportunities. We think that there should be a different system design for GAT. So we did not implement our method for GAT.


Due to space constraints, we omitted the details of some methods. 


For node 4 in Figure 4(c), transferring before aggregation reduces redundant communication (as node 4 can represent the cut edge it is affiliated with). Similarly, node 2 can represent the cut edge it is affiliated with, so aggregation must be done before transferring.


We mapped one MPI process to one CPU NUMA node and one thread to one physical core. There are two MPI processes per Intel node as DistGNN configures and four MPI processes per Arm node


For example, for the UK dataset, due to graph characteristics, the time spent on the local computation is small, which limits the scalability.

We think this fluctuation is within the normal range. 

Since not all neighbors' information is useful for nodes, FP32 neighbors may introduce noise. Converting these neighbors to int2 might reduce the noise they introduce, potentially improving the model's accuracy.

In areas like CFD, much larger graphs (e.g., GraphCast for weather forecasting) exist, which require a scalable GNN system.


Communication optimization is generally applicable to both GPUs and CPUs. In the Related Work section, we summarized the communication optimization approaches proposed by existing GPU and CPU systems. 



In our performance comparison, we aim to select systems that accelerate distributed full-batch training, particularly those that have demonstrated scalability on large-scale machines, as baselines. However, many systems are optimized for mini-batch training, or aim at reducing memory (at small scale), or only show scalability on a small number of machines. Additionally, the GPU systems are based on GPU kernels, so they cannot run on CPUs. In Section 5.8, we just designed a small experiment with the SoTA GPU method BNS-GCN that has demonstrated large-scale scalability in their experiment. BNS-GCN samples boundary nodes, retaining only 10% for communication, making it highly effective for communication optimization. For the distributed full-batch CPU systems, DistGNN is the SoTA system and representative. It is proposed by Intel lab, optimizes operators for Intel CPUs, highly optimizes communication, and shows large-scale scalability for Intel CPU clusters. Additionally, the flow of DistGNN is similar to ours, from single-node to multi-node optimization, making it a fair SoTA fairline.

For fairness and generalization, we set the same model hyperparameters. 


**Q**: Evaluate a broader range of GCN models such as GCN, GAT and GIN

**A**: We tested the accuracy and performance of our method on GCNs during experiments but didn't put them in this paper due to space limits.

**Q**: Why it is superior to delay aggregation if the source node is in the minimum vertex cover.

**A**: Our pre-post-aggregation approach does not reduce in the feature dimension but rather focuses on reducing the number of boundary nodes (cut-edges). 


**Q**: Is the single-node configuration consistent for both Intel and ARM platforms in Figures 6-7?

**A**: Yes.


**Q**: In Table 3, why does the training accuracy fluctuate apparently when the training scale changes?

**A**: Similar fluctuations were also observed in the accuracy results of the previous SoTA works like AdapQ (Table 4). We attribute the fluctuation in our result to the initialization of model parameters and the different distribution of labels incurred by graph partitioning. 


**Q**: How SIMD instruction is leveraged during quantization and dequantization on both X86 and Arm CPUs.

**A**: Since PyTorch Tensor supports only int8 datatype, we pack four int2 elements from different embeddings into one int8 element. we use SIMD instructions to quantize data into int32 and truncate them into int2 based on the scheme. The dequantization process reverses the steps of quantization.


The scalability in our paper refers to strong scaling. When scaling to a certain number of machines, the scalability is limited by the size of the graph, graph characteristics, and the graph partitioning result, which prevents further scalability beyond that point.


It is only because SuperGCN applies extensive optimizations at the single-node level (for computation), that the bottleneck becomes mostly communication.

Many systems, however, are optimized for mini-batch training, memory reduction, or small-scale setups, with GPU-based methods limited to GPUs. 


It is only because SuperGCN applies extensive optimizations at the single-node level (for computation), that the bottleneck becomes mostly communication.


The original memory access is c0->c1->c2->c3->e0->e1... in figure 3(b). We use loop reordering to do the cache (register) tiles to reduce memory access on dst. After loop reordering, the memory access is c0->c1->e0->e1->c2->c3->... 

Our work is the first to use pure int2 for communication and to demonstrate that label propagation can recover the accuracy loss caused by int2 communication.

==> tables/accuracy_IGB260M.tex <==
%Test accuracy (\%) on ogbn-products, Reddit and ogbn-papers100M \zhuang{and validated accuracy (\%) on ogb-lsc-mag240M (no available test label)}. 
\begin{table}
    \centering
        \caption{Final test accuracy of IGB260M on Fugaku. W/o LP refers to training without label propagation, while w/ LP refers to training with label propagation.}
        \resizebox{0.9\linewidth}{!}{  
    \begin{tabular}{|l|c|c|}
        \hline
        \textbf{Method} & 4096 procs & 8192 procs \\ 
        \hline
        % \hline
        \textsf{SuperGCN (FP32, w/o LP)} & 54.90 & 54.89 \\
        % \hline
        \textsf{SuperGCN (Int2, w/o LP)} & \textbf{54.96} & \textbf{54.96} \\
        \textsf{SuperGCN (FP32, w/ LP)} & 54.39 & 54.37 \\
        \textsf{SuperGCN (Int2, w/ LP)} & 54.68 & 54.92 \\
        \hline
    \end{tabular}
    }
    \label{table/experiment:accuracy_IGB260M}
\end{table}

==> tables/comparison_with_gpu.tex <==
\begin{table}
      \caption{Performance comparison with the GPUs method BNS-GCN. $p$ is the ratio of boundary nodes for communication \zhuang{(graph structure changes with a lower $p$)}. BNS-GCN uses 192 Nvidia V100 GPUs vs. SuperGCN on 192 Fujitsu A64FX CPUs. The dataset is Ogbn-papers100M.}        
      %\normal
      \centering
      %\vspace{-10pt}
      \setlength{\tabcolsep}{4mm}
       \resizebox{0.8\linewidth}{!}
       {
          \begin{tabular}{ |l|c| }
          \hline
          \bf{Method} & \bf{Seconds / Epoch}  \\
          \hline
          \textsf{BNS-GCN ($p=1.0$)} & 5.541 \\
          \textsf{BNS-GCN ($p=0.1$)} & 0.587 \\
          \textsf{\zhuang{SuperGCN (w/o comm opt.)}} & 2.163 \\
          \textsf{\zhuang{SuperGCN (w/ comm opt.)}} & 0.823 \\
          % \hline
          % Ogbn-papers100M & 111,059,956 & 1,615,685,872 & 128 & 72 \\
          \hline
           \end{tabular}  
        }
        
       \label{table/experiment:comparison_with_gpu} 
       % }
\end{table}     

==> tables/datasets.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table}
      \caption{The graph datasets used in experiments.}        
      \small
      \centering
      %\vspace{-10pt}
      \resizebox{\linewidth}{!}{
          \begin{tabular}{ |l|c|c|c|c| }
          \hline
          \bf{Datasets} & \bf{\#Vertex} & \bf{\#Edges} & \bf{\#Feat} & \bf{\#Class} \\
          \hline
          \textsf{Ogbn-arxiv} & 169,343 & 1,166,243 & 128 & 40 \\
          % \hline
          \textsf{Reddit} & 232,965 & 114,615,892 & 602 & 41 \\
          % \hline
          \textsf{Ogbn-products} & 2,449,029 & 61,859,140 & 100 & 47 \\
          % \hline
          \textsf{Proteins} & 8,745,542 & 1,309,240,502 & 128 & 256 \\
          % \hline
          \textsf{Ogbn-papers100M} & 111,059,956 & 1,615,685,872 & 128 & 172 \\
          % \hline
          \zhuang{\textsf{Ogb-lsc-mag240M$^{*}$}} & 121,751,666 & 2,593,241,212 & 768 & 153 \\
          \textsf{UK-2007-05} & 105,896,555 & 3,738,733,648 & 128 & 172 \\
          % \hline
          % Ogbn-papers100M & 111,059,956 & 1,615,685,872 & 128 & 72 \\
          \hline
          \multicolumn{4}{l}{$^{*}$We extract the undirected homogeneous papers citation graph.}
           \end{tabular}  
        }
       \label{table/experiment:dataset} 
\end{table}     
%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/models.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table*}
      \caption{The GraphSAGE model hyperparameters used in experiments.}        
      \small
      \centering
      %\vspace{-10pt}
      \resizebox{\linewidth}{!}{
          \begin{tabular}{ |l|c|c|c|c|c|c|c|c| }
          \hline
          \bf{Datasets} & \bf{\#Layers} & \bf{\#Hidden} & \bf{\#Epochs} & \bf{Norm} & \bf{Dropout} & \bf{Learning Rate} & \bf{Weight Decay} & \bf{Aggr Type} \\
          \hline
          \textsf{Reddit} & 3 & 256 & 250 & LayerNorm & 0.5 & 0.01 & 0.0 & Mean \\
          % \hline
          \textsf{Ogbn-products} & 3 & 256 & 250 & LayerNorm & 0.5 & 0.01 & 0.0 & Mean \\
          % \hline
          \textsf{Proteins} & 3 & 256 & 200 & LayerNorm & 0.5 & 0.01 & 0.0 & Mean \\
          % \hline
          \textsf{Ogbn-papers100M} & 3 & 64 & 200 & LayerNorm & 0.5 & 0.01 & 0.0 & Mean \\
          % \hline
          % \textsf{UK-2007-05} & 3 & 128 & 200 & LayerNorm & 0.5 & 0.01 & 0.0 & Mean \\
          \zhuang{\textsf{Ogbn-mag240M}} & 3 & 256 & 300 & LayerNorm & 0.5 & 0.005 & 0.0 & Mean \\
          % \hline
          % Ogbn-papers100M & 111,059,956 & 1,615,685,872 & 128 & 72 \\
          \hline
           \end{tabular}  
        }
       \label{table/experiment:model} 
\end{table*}     
%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/models_small.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table}
      \caption{The GraphSAGE model hyperparameters used in experiments.}        
      \small
      \centering
      %\vspace{-10pt}
      \resizebox{\linewidth}{!}{
          \begin{tabular}{ |l|c|c|c|c|c|c| }
          \hline
          \bf{Datasets}  & \bf{\#Hidden} & \bf{\#Epochs} & \bf{Dropout} & \bf{Learning Rate} \\
          \hline
          \textsf{Reddit} & 256 & 250 & 0.5 & 0.01 \\
          % \hline
          \textsf{Ogbn-products} & 256 & 250 & 0.5 & 0.01 \\
          % \hline
          \textsf{Proteins} & 256 & 200 & 0.5 & 0.01 \\
          % \hline
          \textsf{Ogbn-papers100M} & 64 & 200 & 0.5 & 0.01 \\
          % \hline
          % \textsf{UK-2007-05} & 3 & 128 & 200 & LayerNorm & 0.5 & 0.01 & 0.0 & Mean \\
          \zhuang{\textsf{Ogb-lsc-mag240M}} & 256 & 300 & 0.5 & 0.005 \\
          \textsf{UK-2007-05} & 128 & 200 & 0.5 & 0.01 \\
          % \hline
          % Ogbn-papers100M & 111,059,956 & 1,615,685,872 & 128 & 72 \\
          \hline
           \end{tabular}  
        }
       \label{table/experiment:model_small} 
\end{table}     
%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/performance_IGB260M.tex <==
%Test accuracy (\%) on ogbn-products, Reddit and ogbn-papers100M \zhuang{and validated accuracy (\%) on ogb-lsc-mag240M (no available test label)}. 
\begin{table}
    \centering
        \caption{Performance (seconds per epoch) of IGB260M on Fugaku. \textit{SuperGCN (w/o comm opt)} is our implementation before applying the proposed distributed-level optimization methods, and \textit{SuperGCN (w/ comm opt)} includes all the proposed distributed-level optimization methods.}
        \resizebox{0.95\linewidth}{!}{  
    \begin{tabular}{|l|c|c|}
        \hline
        \textbf{Method} & 4096 procs & 8192 procs \\ 
        \hline
        % \hline
        \textsf{SuperGCN (w/o comm opt)} & 12.40 & 7.62 \\
        % \hline
        \textsf{SuperGCN (w/ comm opt)} & 2.25 & 1.79 \\
        \hline
    \end{tabular}
    }
    \label{table/experiment:performance_IGB260M}
\end{table}
